Solving Royal Game of Ur Using Reinforcement Learning

Reinforcement Learning has recently surfaced as a very powerful tool to solve complex problems in the domain of board games, wherein an agent is generally required to learn complex strategies and moves based on its own experiences and rewards received. While RL has outperformed existing state-of-the-art methods used for playing simple video games and popular board games, it is yet to demonstrate its capability on ancient games. Here, we solve one such problem, where we train our agents using different methods namely Monte Carlo, Qlearning and Expected Sarsa to learn optimal policy to play the strategic Royal Game of Ur. The state space for our game is complex and large, but our agents show promising results at playing the game and learning important strategic moves. Although it is hard to conclude that when trained with limited resources which algorithm performs better overall, but Expected Sarsa shows promising results when it comes to fastest learning.

==> mybib.tex <==
\bibitem{b15}Ganger, M., Duryea, E. \& Hu, W. Double Sarsa and Double Expected Sarsa with Shallow and Deep Learning. {\em Journal Of Data Analysis And Information Processing}. \textbf{4}, 159-176 (2016)
\bibitem{b2}Montague, P., Dayan, P. \& Sejnowski, T. A framework for mesencephalic dopamine systems based on predictive Hebbian learning. {\em The Journal Of Neuroscience}. \textbf{16}, 1936-1947 (1996,1)
\bibitem{b1}Schultz, W., Dayan, P. \& Montague, P. A Neural Substrate of Prediction and Reward. {\em Science}. \textbf{275}, 1593-1599 (1997)
\bibitem{b6}Schultz, W. Predictive Reward Signal of Dopamine Neurons. {\em Journal Of Neurophysiology}. \textbf{80}, 1-27 (1998)
\bibitem{b16}Seijen, H., Hasselt, H., Whiteson, S. \& Wiering, M. A theoretical and empirical analysis of Expected Sarsa. {\em 2009 IEEE Symposium On Adaptive Dynamic Programming And Reinforcement Learning}. (2009)
\bibitem{b5}Sejnowski, T., Dayan, P. \& Montague, P. Predictive Hebbian learning. {\em Proceedings Of The Eighth Annual Conference On Computational Learning Theory - COLT 95}. (1995)
\bibitem{b7}Smith, A., Li, M., Becker, S. \& Kapur, S. Dopamine, prediction error and associative learning: A model-based account. {\em Network: Computation In Neural Systems}. \textbf{17}, 61-84 (2006)
\bibitem{b10}Sturtevant, W. Board and Table Games from Many Civilizations . R. C. Bell.. {\em American Anthropologist}. \textbf{63}, 1396-1396 (1961)
\bibitem{b8}Tan, M. Multi-Agent Reinforcement Learning: Independent vs. Cooperative Agents. {\em Machine Learning Proceedings 1993}. pp. 330-337 (1993)
\bibitem{b4}Montague, P. \& Sejnowski, T. The predictive brain: temporal coincidence and temporal order in synaptic learning mechanisms.. {\em Learning & Memory}. \textbf{1}, 1-33 (1994)
\bibitem{b3}Montague, P., Dayan, P., Nowlan, S., Pouget, A. \& Sejnowski, T. Using aperiodic reinforcement for directed self-organization during development. {\em Advances In Neural Information Processing Systems}. pp. 969-976 (1993)
\bibitem{b9}Brockman, G., Cheung, V., Pettersson, L., Schneider, J., Schulman, J., Tang, J. \& Zaremba, W. Openai gym. {\em ArXiv Preprint ArXiv:1606.01540}. (2016)
\bibitem{b11}Finkel, I. On the rules for the Royal Game of Ur. {\em Ancient Board Games In Perspective. British Museum Press, London}. pp. 16-32 (2007)
\bibitem{b12}He, S. Deep Reinforcement Learning-of how to win at Battleship. {\em CCRi}. (2018,7), http://www.ccri.com/2017/08/25/deep-reinforcement-learning-win-battleship/
\bibitem{b13}Watkins, C. \& Dayan, P. Q-learning. {\em Machine Learning}. \textbf{8}, 279-292 (1992)
\bibitem{b14}Konen, W. Reinforcement Learning for Board Games: The Temporal Difference Algorithm.  (2015)
\bibitem{rlbook}Sutton, R. \& Barto, A. Reinforcement learning: An introduction. (MIT press,2018)
\bibitem{atari}Mnih, V., Kavukcuoglu, K., Silver, D., Rusu, A., Veness, J., Bellemare, M., Graves, A., Riedmiller, M., Fidjeland, A., Ostrovski, G. \& Others Human-level control through deep reinforcement learning. {\em Nature}. \textbf{518}, 529 (2015)
\bibitem{go}Silver, D., Huang, A., Maddison, C., Guez, A., Sifre, L., Van Den Driessche, G., Schrittwieser, J., Antonoglou, I., Panneershelvam, V., Lanctot, M. \& Others Mastering the game of Go with deep neural networks and tree search. {\em Nature}. \textbf{529}, 484 (2016)
\bibitem{b17}Ghory, I. Reinforcement learning in board games. {\em Department Of Computer Science, University Of Bristol, Tech. Rep}. pp. 105 (2004)
\bibitem{b18}Tesauro, G. Td-gammon: A self-teaching backgammon program. {\em Applications Of Neural Networks}. pp. 267-285 (1995)
\bibitem{b19}Tesauro, G. Temporal difference learning and TD-Gammon. {\em Communications Of The ACM}. \textbf{38}, 58-68 (1995)
\bibitem{b20}Schraudolph, N., Dayan, P. \& Sejnowski, T. Temporal difference learning of position evaluation in the game of Go. {\em Advances In Neural Information Processing Systems}. pp. 817-824 (1994)

